Physics-Grounded Motion Forecasting via Equation Discovery for Trajectory-Guided Image-to-Video Generation

Recent advances in diffusion-based and autoregressive video generation models have achieved remarkable visual realism. However, these models typically lack accurate physical alignment, failing to replicate real-world dynamics in object motion. This limitation arises primarily from their reliance on learned statistical correlations rather than capturing mechanisms adhering to physical laws. To address this issue, we introduce a novel framework that integrates symbolic regression (SR) and trajectory-guided image-to-video (I2V) models for physics-grounded video forecasting. Our approach extracts motion trajectories from input videos, uses a retrieval-based pre-training mechanism to enhance symbolic regression, and discovers equations of motion to forecast physically accurate future trajectories. These trajectories then guide video generation without requiring fine-tuning of existing models. Evaluated on scenarios in Classical Mechanics, including spring-mass, pendulums, and projectile motions, our method successfully recovers ground-truth analytical equations and improves the physical alignment of generated videos over baseline methods.

==> sections/Introduction.tex <==

% Given an observed input video, we first extract object motion trajectories using CoTracker. These trajectories are then used to learn motion equations via symbolic regression, enhanced with our retrieval-based pre-training mechanism. The learned equations are used to forecast future object trajectories, which are subsequently used to guide a video generation model, enabling physics-adherent video forecasting.

Recent advances in video generation models have significantly improved the realism of synthesized videos, driven primarily by diffusion-based and autoregressive models \cite{blattmann2023stable, yang2025cogvideox, nvidia2025cosmosworldfoundationmodel, kong2025hunyuanvideosystematicframeworklarge}. These models are capable of generating high-fidelity videos across diverse prompts and scenarios. However, despite visual realism, they often lack physical alignment, failing to reproduce object motion consistent with real-world physical dynamics \cite{kang2024farvideogenerationworld, motamed2025generativevideomodelsunderstand, wang2025wisaworldsimulatorassistant}. This limits their applicability in domains where physical accuracy is essential, such as scientific simulation, robotics, and education.

Some existing video generation models guide the object motion by text prompt \cite{yang2025cogvideox, nvidia2025cosmosworldfoundationmodel, kong2025hunyuanvideosystematicframeworklarge}. However, the text prompt is inherently imprecise, which lacks the specific description of underlying physical dynamics, such as how velocity and displacement vary over time. Other works guide motion using explicit trajectories in the form of $(x,y)$ coordinate sequences \cite{10.1007/978-3-031-72670-5_19, 10.1145/3641519.3657518, namekata2025sgiv, zhang2024toratrajectoryorienteddiffusiontransformer, klingai}. While these models allow some degree of motion control, the trajectories are manually drawn, which makes it difficult to ensure physical correctness, especially for complex motions such as fluid and double pendulum systems, where hand-crafted trajectories may deviate significantly from the true dynamics. 
% Moreover, unlike physics simulators that strictly follow the trajectories, trajectory-guided video generation models do not strictly align to the input trajectory, further limiting their physical fidelity.

One key reason for the lack of physical alignment in current video generation models is their reliance on learning statistical correlations rather than causal mechanisms (\ie physical dynamics). Whether text-driven or trajectory-guided, these models are typically trained on large-scale video datasets to capture patterns in appearance and motion without explicitly modeling the underlying physical dynamics. As a result, they lack an explicit understanding of physical laws such as inertia, gravity, force interactions, and their relations. This reliance on correlation over causation makes it difficult for these models to produce motion that aligns with physical dynamics \cite{motamed2025generativevideomodelsunderstand}.

% One reason of physics misalignment is that current video generation models—whether text-driven or trajectory-guided—are predominantly trained to capture statistical correlations in large-scale video datasets rather than to model causal mechanisms (\ie physical dynamics). As a result, they lack an explicit understanding of physical laws such as inertia, gravity, force interactions, and their relations, which are structured causal relations \cite{Johansson2021}. This reliance on correlation over causation makes it difficult for these models to produce motion that aligns with physical dynamics \cite{motamed2025generativevideomodelsunderstand}.

%For example, it may describe spring mass systems as ``The spring and the attached object move from right to left, gradually slowing down until coming to a complete stop."


To address physical misalignment, we propose a novel video forecasting framework that learns equations of motion from past video and uses them to guide physics-aligned future video forecasting. Our framework integrates symbolic regression (SR) with trajectory-guided image-to-video (I2V) models and operates in a training-free manner. As illustrated in Figure~\ref{fig:overall_pipeline}, we first extract object motion trajectories from past videos, then apply SR, which is enhanced with a novel \textit{\textbf{re}trieval-based pre-training mechanism} (denoted as \ourmethod), to discover equations that govern the motion. These learned equations are used to forecast future trajectories, which serve as control signals for trajectory-guided video generation models. Notably, our framework is \textit{model-agnostic}, making it compatible with any trajectory-conditioned I2V model without additional fine-tuning.

To ground our study in a tractable setting, we focus on a class of videos where: 1) object motion is constrained to a 2D plane and captured from an orthographic viewpoint; 2) trajectories are fully observable throughout the video; and 3) the scenes depict classical physics systems such as spring-mass, pendulums, and projectile motion. While this scope may appear narrow, it includes a broad range of real-world applications—including physics education, scientific visualization, physics simulation, and virtual experimentation. Moreover, it provides a controlled environment where physical alignment can be quantitatively assessed, serving as a foundation for future work in more complex and generalizable settings.

Our contributions are summarized as follows:
\begin{itemize}
    \item We propose a novel framework for training-free, physics-aligned video forecasting, which combines SR with trajectory-guided video synthesis. Our approach operates entirely at inference time and does not require fine-tuning of video generation models.
    \item We introduce a \textit{retrieval-based pre-training mechanism} for SR, denoted as \ourmethod, which significantly improves convergence speed and accuracy in learning equations from observed trajectories.
    \item We demonstrate that \ourmethod effectively discovers equations that closely match both ground-truth analytical equations and observed trajectories. Moreover, our video forecasting framework achieves better physical alignment compared to existing baselines.
\end{itemize}






% {\bf [TT:]
% Besides the motivation (existing video generation does not follow physics), in the introduction, we may need to narrow down our scope of video forecasting to certain types of video content, observed motion is assumed to be perpendicular to the orthogonal (non-perspective) camera, ignoring the perspective viewing transformation, and occlusion-free, etc.

% Then we will have to justify why this narrow-down scope remains useful in our application.
% }

% \tao{video scope, focus on physics systems in lab environment, also in title; equation of motion or equation of dynamics system. Without trajectory (obtain from equation), current model predict future conditioned on one image or text prompt, which make models to predict based on correlation. Or use human draw trajectory, which is based on human intuition (feeling) without real computation still based on correlation. }

